Forecasting Financial Market Structure from Network Features using Machine Learning

We propose a model that forecasts market correlation structure from link- and node-based financial network features using machine learning. For such, market structure is modeled as a dynamic asset network by quantifying time-dependent co-movement of asset price returns across company constituents of major global market indices. We provide empirical evidence using three different network filtering methods to estimate market structure, namely Dynamic Asset Graph (DAG), Dynamic Minimal Spanning Tree (DMST) and Dynamic Threshold Networks (DTN). Experimental results show that the proposed model can forecast market structure with high predictive performance with up to $40\%$ improvement over a time-invariant correlation-based benchmark. Non-pair-wise correlation features showed to be important compared to traditionally used pair-wise correlation measures for all markets studied, particularly in the long-term forecasting of stock market structure. Evidence is provided for stock constituents of the DAX30, EUROSTOXX50, FTSE100, HANGSENG50, NASDAQ100 and NIFTY50 market indices. Findings can be useful to improve portfolio selection and risk management methods, which commonly rely on a backward-looking covariance matrix to estimate portfolio risk.

==> literature.tex <==

\section{Stock Market Structure and Network Prediction}

(UNDER REVIEW)

In~\cite{Mantegna1999}, the authors introduce one of the most commonly used methods to perform structure and topological analysis of financial markets, where assets are represented as nodes and edges represent the relationship between assets based on correlation measures between time series of log-returns of assets. It is used in several studies, including~\cite{gopikrishnan2000scaling},~\cite{onnela2003dynamics},~\cite{lee2012overall},~\cite{bonanno2003topology},~\cite{bonanno2004networks} and~\cite{eom2009topological}. In~\cite{onnela2004clustering}, the authors discuss how to select the relevant correlations through the correlation matrix among stocks and compare the results with random graphs. In addition to Pearson's correlation~\cite{feller1968introduction}, the most popular approach to measure the correlation between two assets, other approaches have been investigated to extract the market structure. In~\cite{yang2014cointegration}, the authors investigate the construction of financial networks using co-integration coefficient between the main indices of world financial markets~\cite{granger1981some}~\cite{johansen1990maximum}. In~\cite{tabak2010topological}, topological properties of financial networks in the Brazilian stock market are assessed using a Minimum Spanning Tree algorithm, employing correlation matrix of the asset price variation of several sectors. These studies often describe the stock market structure using graphs~\cite{bonanno2004networks}~\cite{lee2012overall}. In~\cite{spelta2017financial}, the author proposed a method to predict abrupt market changes by inferring the forthcoming dynamic of stock prices through the prediction of future distances between them, using a tensor decomposition technique. Other areas, besides stock market, use time series transformation in complex networks for different analyzes, such as time series clustering~\cite{ferreira2016time} and time-series link prediction~\cite{Yang2008}.

Another subject related to this work is the stock market structure prediction. We addressed this problem as a link prediction task. For such,
%It consists of using 
previously known network information is used to find connections that may appear in the future or simply to find hidden connections. This predictive task is investigated 
%difficult task is the main objective of researchers 
in many real problems, mainly involving social networks~\cite{martinez2017survey}~\cite{grover2016node2vec}. Some authors separate the type of link prediction according to the method, like similarity-based methods, probabilistic and statistical methods, and algorithmic methods, which include methods based on Machine Learning (ML)~\cite{marti2017review}. Other authors differentiate the type of prediction according to the specific nature of the problem, such as dynamic link prediction or hidden link prediction, as well as the application of link prediction, such as recommendation in social networks or network completion~\cite{wang2015link}. ML based methods treat the link prediction problem as a binary classification task, whose classes are linked and not linked. In~\cite{al2006link}, the authors investigate the use ML to identify possible links in future networks. In~\cite{da2012time}, the authors investigate the prediction of links using time series forecasting over similarity metrics. 

In a real stock market scenario, relationship between assets can not only appear along the time, but can also disappear. Thus, assets can have dynamic interactions. A sequence of dynamic interactions over time introduces another dimension to the challenge of mining and predicting link structure, named temporal link prediction~\cite{dunlavy2011temporal}. Temporal networks are a specific type of dynamic networks in which time can be organized as a third-order tensor, or multi-dimensional array~\cite{wang2015link}.
A common deficiency of these methods is keeping the links between nodes even when their relationship no longer exist. 
To address this deficiency, we propose a model to predict future market correlation structure using link- and node-based financial network features, differing from the previous studies mainly regarding to the possibility of identifying removal of links over the time. 
